Particle Physics at the European Spallation Source

Presently under construction in Lund, Sweden, the European Spallation Source (ESS) will be the world's brightest neutron source. As such, it has the potential for a particle physics program with a unique reach and which is complementary to that available at other facilities. This paper describes proposed particle physics activities for the ESS. These encompass the exploitation of both the neutrons and neutrinos produced at the ESS for high precision (sensitivity) measurements (searches).

==> HIBEAM_obsolete.tex <==
\section{HIBEAM}\label{sec:nnprimesearches}

HIBEAM is focused on searches for sterile neutrons and the performance of a pilot experiment for a future high precision search for free neutrons transforming to antineutrons (see Section~\ref{sec:nnbar}. The program is based on experiments which can be performed for relatively short times using the ANNI beamline \textit{without} full ESS power. These searches are described below. 

\subsection{Search for $n \rightarrow n{'}$ via disappearance}\label{sec:nnprime} Neutron ($n \rightarrow \{n{'},\bar{n}'\}$) is sensitive to a scenario in which at least one of the mixing parameters $\alpha_{nn'}$ or $\beta_{n\bar{n}'}$ (see Eq.~\ref{eq:nbarmatrix}) is non-zero. The presence of an unknown sterile magnetic field $\mathbf{B{'}}$ is taken into account by performing a magnetic field scan such that the sterile and visible magnetic fields are matched and a $n \rightarrow n{'}$ transition is less suppressed.
  
 Neutrons would move through an aluminum vacuum tube. The tube has a length of around 50m. Neutron rates at the start and the end of the propagation must be measured precisely. 
 
 %An assumption is made that the sterile magnetic field is constant, uniform, and less than the magnitude of the Earth's magnetic field \cite{Berezhiani:2008bc}. The variation of neutron flux will be made axial laboratory magnetic field values in different directions in the interval $-0.5$G to $+0.5$G with steps corresponding to a few mG which is much smaller than the resonance-width. The counting rate will be controlled by the magnitude of magnetic field. 

The detection of a resonance would manifest itself as a reduction in the total counting rate. A discovery or limit on the mass mixing parameter $\epsilon$, or the $n \rightarrow n{'}$ oscillation time $\tau_{n\rightarrow n'}^{dis}$, can be extracted. A positive signal would be of fundamental significance in establishing the existence of a sterile sector.  More detailed scans could be used to determine the 3-dimensional direction of the sterile magnetic field.
%In case of no resonance detected in the counting rate ratio $C/M$, a limit will be set on the $n \rightarrow n{'}$ oscillation time $\tau_{n\rightarrow n'}^{dis}$. 

The search for $n \rightarrow n{'}$ via the disappearance mode requires full magnetic control in the flight region in the vacuum tube. The 3D 
magnetic field must be approximately uniform and be set to a given 3D field value in any direction with an accuracy 2 mG. The scan over magnetic field values should take place between 0 mG  to $\sim 500$mG, presenting a technical challenge for this experiment. 

Charge-integrating counters are needed which are able to measure a charge proportional to the $n$ flux with an relative accuracy up to $\order10^{-7}$. %this was true (but marginal) at HFIR but we want much higher accuracy at HIBEAM...
One possibility is the use of a $^3He$ detector ~\cite{doi:10.1063/1.4919412} in charge-integration mode. 

%Searches made with positive and negative $\mathbf{B}$-field directions would allow a determination of the oscillation time $\tau_{n\rightarrow n'}^{dis}$ which is independent of the the value of the unknown angle $\beta$ between the visible and sterile magnetic fields ($\mathbf{B}$ and $\mathbf{B{'}}$, respectively). It can also be used to provide an estimate of the angle $\beta$.

%The sensitivity for oscillation time for low magnetic field disappearance searches in the absence of visible resonance signal depends on the bare and square-normalized integrals of the neutron velocity spectrum~\cite{Berezhiani:2017azg}.

 Signal sensitivity at a $95\%$ CL were estimated. A series of $200$ separate magnetic field point measurements and $25$ background runs were considered.  Equidistributed run folding over a specific magnetic field range (eg $[-200,200]$mG) was made. A background of $1$ n/s and a $30\%$ $n$ monitor efficiency was assumed. The flight path was divided into two $25$m magnetically controlled sections. The oscillation time sensitivity can be calculated for a range of detector radii. One ESS operating year of approximately $200$ days was assumed. The sensitivity of the disappearance search is shown in Fig.~\ref{fig:DisappearanceRegenerationTaus} as a function of detector radii. The sensitivities for the regeneration modes (\ref{sec:regen}) is also shown. Limits from searches at UCN sources~\cite{Ban:2007tp,Serebrov:2009zz,Altarev:2009tg,Berezhiani:2012rq,Berezhiani:2017jkn,Abel:2020kdg} are also presented. 
It can be seen that HIBEAM has sensitivity to a wider range of oscillation times for many regions of magnetic field. Furthermore, a series of searches for $n\rightarrow n'$ conversions for neutrons in flight  are planned at the High Flux Isotope Reactor (HFIR) at Oak Ridge National Laboratory~\cite{Broussard:2017yev,Broussard:2019tgw}. 

\begin{figure}[H]
  \setlength{\unitlength}{1mm}
  \begin{center}
  \includegraphics[width=1.0\linewidth, angle=0]{nnprimelimitsglobal-new.pdf}
  \end{center}
  \vspace{0.0cm}
  \caption{\footnotesize Excluded neutron oscillation times in blue for $n\rightarrow n'$ disappearance from UCN experiments~\cite{Ban:2007tp,Serebrov:2009zz,Altarev:2009tg,Berezhiani:2012rq,Berezhiani:2017jkn,Abel:2020kdg} as a function of the magnetic field $\mathbf{B{'}}$. The projected sensitivity  for HIBEAM (disappearance mode) is also shown in magenta for one year's running at the ESS assuming a power of 1MW.}
  \label{fig:nnprime-global}
\end{figure}


%Whilst it is non-trivial to quantify the reach of other planned searches, a basic description is given here. %standard practice is to include self-reported expected reach, but not needed here

\subsection{Search for the regenerative $n \rightarrow n{'} \rightarrow n$ process}\label{sec:nnprimen}
The regeneration search derives from a similar theoretical basis as the disappearance search 
\cite{Berezhiani:2017azg,Broussard:2017yev}, though corresponding to a two-stage (second order) process with a consequently quadratically smaller probability. In the first stage, the $n \rightarrow n{'}$ transformation takes place in an intense cold $n$ beam at the quasi-free environment limit corresponding to $|\mathbf{B}-\mathbf{B{'}}|\sim 0$. The largely untransitioned $n$ beam will be blocked by a high suppression beam trap, while the remaining sterile $n'$ will continue unabated through the absorber; in a second volume behind the absorber (stage two), maintainig the the same conditions of $|\mathbf{B}-\mathbf{B{'}}|\sim 0$ as the section before it, the $n{'} \rightarrow n$ transformation produces detectable $n$'s with momentum conserved, as though the totally-absorbing wall were not present at all. The resonance-behaviour depends primarily on the magnitude of the laboratory $\mathbf{B}$; if the vectors of $\mathbf{B}$ and $\mathbf{B{'}}$ are not well aligned, i.e. the angle $\beta \not\approx 0$, the oscillation can still occur with somewhat reduced amplitude \cite{Berezhiani:2008bc}. This fe08:30ature provides a robust systematic check for the experiment: oscillations can be turned off simply by changing the magnitude of $\mathbf{B}$ out-of-resonance in the volume before and/or after absorber. Taking measurements at the positive and negative magnitudes of the field $\mathbf{B}$ in both volumes (four combinations) allows for a determination of the oscillation time independent of the angle $\beta$.

\begin{figure}[H]
  \setlength{\unitlength}{1mm}
  \begin{center}
  \includegraphics[width=0.90\linewidth,08:30 angle=0]{RegenerationwithBackgrounds_NEWEST.png}
  \end{center}
  \caption{\footnotesize Sensitivity at $95\%$ CL on the oscillation time as a function of the apparent background count for regeneration searches, $\tau_{n\rightarrow n'\rightarrow n}$ and $\tau_{n\rightarrow \bar{n}'\rightarrow n}$, in a low magnetic field configuration after $50$m of flight shown for a $0.5$m radius detector for the nominal 1MW HIBEAM/ANNI flux.}
  \label{fig:RegenerationBackgrounds}
\end{figure}

The observation of the resonance in the $\mathbf{B}$-scan would be defined by a sudden appearance of regenerated $n$'s when the $\mathbf{B}-\mathbf{B{'}} \approx 0$ condition in both volumes is met. Like with disappearance, a positive signal would be a demonstration of the $n{'}\rightarrow n$ transformation as well as the existence of the sterile $n'$ and $\gamma{'}$. The requirement of matching conditions in both volumes ensures this type of measurement is significantly more robust to systematic uncertainties that could cause a false signal to be observed, and provides an unambiguous test of that hypothesis.



\begin{figure}[H]
  \setlength{\unitlength}{1mm}
  \begin{center}
  \includegraphics[width=1.00\linewidth, angle=0]{RegenerationScheme1.pdf}
  \end{center}
  \caption{\footnotesize A simplified schematic of the $n\rightarrow n{'} \rightarrow n$ and $n\rightarrow \bar{n}' \rightarrow n$  regeneration searches. Two aluminum vacuum tubes with lengths 25 m are shown. The symbol $N$ represents a  low efficiency beam monitor, $R$ shows a $^3$He high-efficiency low-background counter and $S$ is a beam absorber. An axial magnetic field is applied in different directions (shown by up and down arrows within parentheses) in the two vacuum tubes, and the configurations can be alternated to choose between hypothetically identical (opposite) magnetic moments of $n$ and $n'$ ($\bar{n}'$).}
  \label{fig:RegenerationScheme1}
\end{figure}

For the regeneration experiments, in the absence of an observed signal above background level, an upper limit on the oscillation time
$\tau_{n\rightarrow n'}^{reg}$ can be established from a statistical analysis. This limit was parameterized in \cite{Berezhiani:2017azg} through the quartic-normalized integral of the velocity spectrum
\begin{equation}
    J_4 = \int \frac{S(v)}{v^4} dv
\end{equation}
providing the following estimate for the oscillation $n\rightarrow n{'}$ time:

\begin{equation}
    \label{eq:regenerationsensitivity}
    \tau_{n\rightarrow n'}^{reg} > {\left(\sqrt{4T} \cdot \frac{L^4}{4 g \sqrt{\bar{n}_b}} \cdot J_4\right)}^{\frac{1}{4}}
\end{equation}
where $\bar{n}_b$ is the average background rate in the detector $R$ (see Fig. \ref{fig:RegenerationScheme1}) in n/s. This calculation is again based on the single maximum deviation of one of the folded magnetic scan 
of 200 measurements and $T$ is time for one 
individual measurement.
Running over possible values of this background rate, the behavior of the upper oscillation limit can be constructed and is shown in Fig. \ref{fig:RegenerationBackgrounds}. It should be noted that the regeneration mode searches are susceptible to environmental background rates only due to full beam absorption at the halfway-point of the beamline. From Eq. (\ref{eq:regenerationsensitivity}), it can be seen that the length $L$ of each of two vacuum tubes in the regeneration scheme is the only parameter that can essentially increase the limit for $\tau_{n\rightarrow n'}^{reg}$. The regeneration oscillation time sensitivity is lower for the same running time than for the disappearance mode as the former (latter) is a two-transition (single-transition) process. However, both processes are complementary with different experimental configurations and neither sharing the same sets of experimental uncertainties. Furthermore, any observation in the disappearance mode could be verified by a regeneration experiment running for a longer time.

\subsection{Search for $n\rightarrow \bar{n}' \rightarrow n$}\label{sec:regen}
As discussed in Section~\ref{sec:nnprimeform}, the symmetry between ordinary matter and mirror matter in general allows a range of  transformations between the visible and sterile neutron sectors, beyond the simple $n\rightarrow n'$ process which is tackled in Sections~\ref{sec:nnprime} and~\ref{sec:nnprimen}. A neutron can be transformed into a mirror (sterile) antineutron which then regenerates back to a detectable $n$ state: $n \rightarrow \bar{n}{'} \rightarrow n$. Since the angular momentum  of the neutron is conserved, the magnetic moment of the  mirror antineutron will be oppositely aligned to the magnetic moment of the sterile neutron due to the mirror $CPT$ theorem. Therefore, a resonance should be observed when magnetic fields in the first and second flight tubes are opposite in direction. This field configuration is included in the anticipated set of measurements shown in Fig.~\ref{fig:RegenerationScheme1}. This search will therefore be be made as a complement to $n \rightarrow n{'} \rightarrow n$  discussed in Section~\ref{sec:nnprimen} and with a similar sensitivity.
\subsection{Search for $n\rightarrow \bar{n}$  by regeneration through mirror states.} \label{sec:nnprimebarn}

Searches for $n\rightarrow \bar{n}$ assume that the transformation occurs via mixing with a non-zero mass amplitude $\varepsilon_{n\bar{n}}$ term; this necessitates magnetic shielding in a search. However, $n\rightarrow \bar{n}$ can also arise due to the second order oscillation processes: $n\rightarrow n{'}\rightarrow\bar{n}$ and $n\rightarrow \bar{n}{'}\rightarrow \bar{n}$, with an amplitude comprised of $\beta_{n\bar{n}'} \alpha_{nn'}$ and associated interference terms. The earlier body of  searches~\cite{Bressi:1989zd,Bressi:1990zx,Fidecaro:1985cm,BaldoCeolin:1994jz} for free $n\rightarrow \bar{n}$ would be insensitive to this scenario. 

A schematic layout of the search for $n\rightarrow \bar{n}$ through regeneration is shown in Fig.\ref{fig:RegenerationScheme2}. Construction of the $\bar{n}$ annihilation detector at the end of second vacuum volume will be required for this experiment. A search for $n\rightarrow \bar{n}$ through regeneration is complementary to the classic $n\rightarrow \bar{n}$ search assuming no sterile neutron mixing. Discussion of the details of the annihilation detector is therefore deferred to Section~\ref{sec:nnbardet}, where it is described in the context of the classic $n\rightarrow \bar{n}$ search. 
%However, it can be noted here that an efficiency substantially in excess of that achieved at the ILL~\cite{BaldoCeolin:1994jz}) (50\%) for the detection of the annihilation of antineutrons can be expected owing to the use of more modern detector techniques. 

\begin{figure}[H]
  \setlength{\unitlength}{1mm}
  \begin{center}
  \includegraphics[width=1.00\linewidth, angle=0]{RegenerationScheme2.pdf}
  \end{center}
  \caption{\footnotesize A $n\rightarrow \{n{'},\bar{n}'\} \rightarrow \bar{ n}$ regeneration search schematic using two aluminum vacuum tubes with diameter $1\,$m. The symbol $N$ represents a low efficiency beam monitor, $A$ shows an annihilation tracking detector enclosing a carbon foil target to capture the annihilation $\bar{n}C$ event, all of which is surrounded by $V$, a cosmic veto system. An axial magnetic field is applied in different directions in the two tubes.}
  \label{fig:RegenerationScheme2}
\end{figure}

\subsection{Complementarity of searches for sterile neutrons generated via mass mixing}
The program of searches has the potential to both make a fundamental discovery of a dark sector and to quantify the processes underpinning the observations. For example, if the search discussed in Section~\ref{sec:nnprime} would detect a signal in the disappearance mode, this would imply a disappearance for all possible final states of oscillating neutrons. Since the magnetic moment of a neutron is oppositely aligned to that of an antineutron due to $CPT$ theorem (and as for sterile neutron and antineutrons), it will be advantageous to use non-polarized beams. Here, the compensation $\mathbf{B\approx B{'}}$ would imply transformations to $\bar{n},n{'},\bar{n}{'}$ for different initial polarization states of neutrons. In regeneration searches, all four magnetic field combinations in two flight volumes would be possible, with $\mathbf{\pm B_1}$ versus $\mathbf{\pm B_2}$ used to detect all possible channels of $n\rightarrow$ regeneration and $n\rightarrow \bar{n}$ due to mass mixing amplitudes $\alpha_{nn'}$ and $\beta_{n\bar{n}'}$.


%\vspace{2 pt}
\subsection{Search for regeneration through a neutron transition magnetic moment (gradients method)}\label{sec:nprimetmmgrad}

As discussed in Section~\ref{sec:nnprimeform} and shown in Eq.~\ref{eq:nnprimetimm}, the probability of the process $n\leftrightarrow n'$ due to a TMM with magnitude $\kappa$ for sufficiently large magnetic fields is approximately  constant,  $P_{n'} = {\kappa}^2$. Due to the independence of $P_{n'}$ on the magnitude of magnetic fields, the oscillating $(n,n')$ system can travel through strong magnetic fields while retaining the same probability of transformation. In a classical sense, the gradients of the magnetic field potential $\mathbf{\mu} \cdot \mathbf{B(r)}$ cause a force acting only upon the neutron part of the $(n,n')$ system, but \textit{not} on the sterile neutron part. Thus, the components of $(n,n')$ system are separated in space as with two spin components in a Stern-Gerlach experiment. When passing through a difference of magnetic potential, the difference in kinetic energies of the $(n,n')$ components can become larger than the energy-width of the wave packet of the system: this ``measures'' the system by collapsing it into either a pure $n$ or pure $n'$ state. The required magnetic field gradient corresponding to the ``measurement'' event can be found according to 
\cite{Berezhiani:2018qqw} from the following equation:
\begin{equation}
    \label{eq:gradient}
 \frac{\Delta B}{\Delta x}>\frac{1}{\mu v (\Delta t)^2}=\frac{v}{\mu (\Delta x)^2},
\end{equation}
where $\Delta x$ is the distance traveled in the magnetic field for time $\Delta t$, $\mu$ is neutron magnetic moment, and $v$ is the neutron velocity.

The presence of strong magnetic field gradients  destroys the ``entanglement'' of the oscillating $(n,n')$ system. A surprising consequence is that as the system continues through the gradient and has its initial state repeatedly reset, this creates additional opportunities for the transformations $n\rightarrow n'$ or $n'\rightarrow n$, effectively increasing the transformation rate. In Ref.~\cite{Berezhiani:2018qqw} this mechanism was suggested as an explanation for the neutron lifetime anomaly~\cite{nlife:2018wfe}. The disappearance of neutrons due to the magnetic gradients present in UCN trap experiments could explain the $\sim 1\%$ lower value of the measured $n$ lifetime in bottle experiments than is seen in measurements using the beam method. This explanation of the $n$ lifetime anomaly together with existing limits from the direct experimental $n\rightarrow n'$ searches implies~\cite{Berezhiani:2018qqw} that $\kappa$ is in the range  of $\sim 10^{-4}-10^{-5}$.

To test this hypothesis, solenoidal coils with alternating currents in each coil can be implemented around the two vacuum tubes to create a magnetic field along the beam axis with a ``zig-zag'' shape, providing an almost constant gradient along the  tube length. These coils can be applied in a regeneration experiment scheme as shown in Fig. \ref{fig:RegenerationScheme1} to search for $n$TMM-induced $n\rightarrow n'\rightarrow n$ regeneration effect with $\kappa < 10^{-5}$. Another opportunity still under development is the use of a cylindrical Halbach array.

%\vspace{5 pt}
\subsection{Search for regeneration through a neutron TMM (compensation method.)}
\label{sec:nprimetmmcom}

As described in \cite{Berezhiani:2018qqw} and Section~\ref{sec:nnprimeform}, an enhanced $n\rightarrow n'$ transformation rate can be produced in a gas atmosphere due to the $n$TMM. A constant magnetic field $\mathbf{B}$ will be applied in the flight volume to give rise to a negative magnetic potential which will compensate the positive Fermi potential of the gas. The gas density should be sufficiently low to avoid incoherent scattering or absorption of the neutrons, resulting in a pure oscillation with probability (from Eq.~\ref{eq:Probc1}) $P_{nn'}=(\epsilon_{nn'}+\kappa \mu B)^2 t^2$. The magnetic field is then scanned in order to search for a resonance condition resulting in a regeneration signal. The magnitude of the laboratory magnetic field at which the resonance might occur depends on the magnitude of the neglected hypothetical sterile magnetic field. The magnitude of $\mathbf{B{'}}$ can be determined by setting the laboratory magnetic field to zero and instead scanning the pressure in the flight tube. In this scenario, the probability is described by the corresponding equation:
\begin{equation}
P_{nn'}=(\epsilon_{nn'} \pm \kappa \mu B{'})^2 t^2
\end{equation}\label{eq:Probc2} where $\pm$ is due to the different possible parities of the sterile magnetic field. Thus, the magnitude of $\mathbf{B{'}}$ can be also independently determined.

\subsection{Neutron detection for sterile neutron searches}
All forms of the sterile neutron searches rely on measurement of the visible state of the neutrons. Detection of cold and thermal neutrons requires major technical competence for the scattering experiments of the ESS, though a standard solution for neutron detection may utilize gas detectors based on \isotope[3]{He} in a single wire proportional chamber. The detectors can be operated at low gain since the $n+\isotope[3]{He}\rightarrow t+p$ reaction produces a very large ionization signal. While this is the baseline technology assumed for HIBEAM, it is also possible that modern readout solutions from high energy physics can augment the performance of such a neutron detection scheme further. As an example, the most challenging readout scenario is considered here, in which each neutron in the flux would be individually detected.  Assuming a neutron flux of $10^{11}\,$n/s evenly spread out over a circular surface of diameter 2m, and assuming each detector element to be about 1 square cm in transverse area, one would have 30000 readout channels with a singles counting rate in each channel of about 3MHz. This rate is indeed not trivial to deal with but it can be accommodated by the ATLAS TRT detector, where each detector element is a single wire proportional chamber (operated at high avalanche gain) read out on the wire. Typical singles counting rates in the ATLAS TRT are in the range of 6--20\,MHz, so 3\,MHz seems quite feasible in comparison.  The ATLAS TRT electronics will be taken out from the ATLAS setup in 2024, presenting a timely opportunity for HIBEAM, and are therefore an interesting possibility to investigate for use in HIBEAM. The energy of the reaction products do not provide any useful information about the originating neutron, therefore only the number of neutrons detected would be recorded in the data stream. The use of coincidence criteria with neighbouring detector cells will also be investigated, to avoid double counting when nuclear fragments leak into neighboring cells. 

If the individual counting of neutrons is not necessary, an integration of the released charge in the detector material gives a measurement proportional to the number of incoming neutrons. After proper calibration, such current integration is less\begin{figure}[!htb]
  \setlength{\unitlength}{1mm}
  \begin{center}
  \includegraphics[width=0.9\linewidth, angle=0]{nnprime-cartoon-new.jpg}
  \end{center}
  \caption{\footnotesize Illustration of the principles of searches for sterile neutron oscillation searches. In the UCN trap (a), it is possible that neutrons effectively disappear, possibly lowering the measured values of the neutron lifetime.  For neutron beams, both disappearance (b) ($n\rightarrow n'$) and regeneration (c) ($n\rightarrow\{\bar{n},n'\}\rightarrow n$) search modes are possible. Another possibility (d) is regenerative in style, though instead leads to further mixing to an antineutron ($n\rightarrow\{\bar{n},n'\}\rightarrow \bar{n}$), requiring an annihilation detector just as shown in Fig. \ref{fig:nnbar-cartoon}. Each regeneration mode requires a neutron absorber to be placed at the halfway point of the beamline, preventing all ordinary neutrons from proceeding downbeam while permitting sterile species to pass unencumbered.}
  \label{fig:nnprime-cartoon}
\end{figure} sensitive to the actual rate of neutrons. It should also be mentioned that, in view of the shortage of \isotope[3]{He}, much R\&D is done for scattering experiments on other methods for cold neutron detection. Synergies with readout systems developed for high energy experiments are expected, and neutron detection in HIBEAM is a good example of an application with a specific scientific use as motivation for exploring such synergies.

==> UCN_old.tex <==
\clearpage
\section{UCN/VCN - 5 pages}\label{sec:ucn}
{\it Hartmut Abele, Klaus Kirch, Egor Lychagin}

%Short intro to UCN. Sections to be augmented for VCN.
The energy of ultracold neutrons (UCNs) is so low ($~10^{-7} eV$) that they can be reflected from many materials at any angle of incidence. This property allows storing UCNs in closed material traps \cite{Zeldovich1959}, and such low energies also make it possible to store them in magnetic traps \cite{Vladimirskii1962}. The possibility of long confinement times (several hundred seconds) for UCNs in experimental setups makes these neutrons extremely sensitive to small effects. In some cases, UCNs turn out to be a more sensitive "instrument" in comparison with thermal and cold neutrons, despite the significantly lower fluxes. The work of F.L. Shapiro \cite{Shapiro1968}, in which he first drew attention to this fact, led to the discovery of UCNs \cite{Luschikov1969,Steyerl:1969csa} and the rapid development of this area of research throughout the 1970s-1990s. It led to a significant improvement in the accuracy of measurements of the neutron lifetime \cite{PDG2020}, constraints on the existence of a neutron electric dipole moment \cite{Abel:2020gbr}, and the discovery and study of UCN quantum states above a flat mirror in a gravitational field \cite{Nes2000}. Since the discovery of UCNs, a great deal of methodological experience has been accumulated in the production, detection, spectrometry, and storage of UCNs. UCN losses on the walls of the storage volumes can be lower than a few percent of the losses associated with neutron decay. Processes involving small energy transfers were also discovered in the interaction of UCNs with material surfaces \cite{Nes1997}, which had not been taken into account in early experiments. It remains a challenge for experimentalists to obtain the theoretically predicted loss factors on weakly-absorbing materials such as solid oxygen and beryllium \cite{Alf1992}. 

Throughout this time, progress in the experimental accuracy was primarily associated with increasing the intensity of UCN sources. However, even today the intensity of the sources is still too low for widespread use of UCNs in surface physics \cite{Golub1996}. The active development of other, relatively cheap methods for studying surfaces seems to indicate that UCN science is not competitive in this area and is unlikely to find application there in the near future -- unless a major advance could be realized in UCN source technology. It therefore seems likely that in coming years, the main area of application for UCNs will remain in the field of particle physics and fundamental interactions.

\subsection{Implementing a UCN source at the ESS}
Delivering higher numbers of UCN into experiments remains the most important possibility to improving experimental accuracy. In certain cases, namely those storage experiments where the free neutron lifetime is not the limiting loss mechanism, significant gains may also be made by increasing the holding time. One should also note that some experiments rely on a high transmitted flux of UCNs, rather than a high stored density. In all cases, however, present-day experiments with UCNs are most strongly limited by counting statistics.

The longest-running and most reliable user-mode UCN source is PF2 at the Institut Laue-Langevin, based on the concept of a Doppler-shifting neutron turbine \cite{pf2_VCN}. All new UCN sources presently under construction use solid deuterium or superfluid helium as superthermal converters for cold neutrons \cite{Golub1975}, \cite{Golub1979}, \cite{Altarev1980}. In contrast to moderation, superthermal conversion increases the out-of-equilibrium UCN phase-space density, via inelastic scattering where a Boltzmann factor suppresses those interactions which lead to an increase of the neutron energy. Both of these converter materials are well studied \cite{Doge:2015cqz}, \cite{Zimmer2014}. Solid deuterium provides a higher conversion rate, where the optimal spectrum for incident neutrons has an effective temperature of $\sim30$~K, and the optimal converter temperature is $\sim5$~K. The high UCN production rate makes this an attractive option for pulsed neutron sources, but absorption losses limit the lifetime of UCNs inside the source. It would be desirable for a UCN source at the ESS to deliver UCN densities limited only by the pulsed neutron flux density. Theoretically, such an approach \cite{Shapiro1970} and its development \cite{Frank1996} was proposed long ago, but to date no known technology can successfully implement this idea. The maximum gain factor in the UCN density for ESS (with a pulse duration of 2.5~ms and a pulse frequency of 14~Hz) would be $\sim30$~ times.

%An advantage of implementing this type of UCN source at the ESS could be the accumulation of UCN densities limited by the pulsed neutron flux density. Theoretically, such an approach \cite{Shapiro1970} and its development \cite{Frank1996} was proposed long ago, but until now no technology is known that can successfully implement this idea. The maximum gain factor in the UCN density for ESS (with a pulse duration of 2.5~ms and a pulse frequency of 14~Hz) is $\sim30$~ times.

Superfluid helium has a rate of UCN production almost 10 times lower, and the optimal spectrum for incident neutrons has an effective temperature of $\sim6$~K. At temperatures below $\sim0.8$~K superfluid helium permits very long UCN lifetimes in the converter (finally limited by beta decay below $\sim0.6$~K), making it possible to accumulate UCNs over long times and obtain high ``\emph{in-situ}" densities within the converter volume. The \emph{in-situ} UCN density $\rho_\text{source}$ will be reduced by dilution and transfer losses, for any extraction-based experiment in which the UCNs are transferred to an \emph{ex-situ} storage volume for measurement. For a perfect guide system in which dilution losses dominate, the density $\rho_\text{expt}$ of UCNs delivered into such an experiment is determined by the volumes of the source ($V_\text{source}$), guide system ($V_\text{guide}$), and experiment ($V_\text{expt}$):

\begin{equation}
    \rho_\text{expt} = \frac{V_\text{source}\rho_\text{source}}{V_\text{source} + V_\text{guide} + V_\text{expt}} .
\end{equation}
The long times required for obtaining the saturated UCN density in a helium converter make it unrealistic to exploit the time-structure of a pulsed neutron source for further gains in UCN density (although the time-structure associated with neutron delivery can be experimentally useful for disentangling beam-related backgrounds). However, since the average thermal neutron flux density expected from the ESS is comparable to the ILL or PIK reactor sources, a helium-based UCN source could run at the ESS without loss in the UCN production rate. In addition the delivery of large-area neutron beams, or use of novel imaging concepts, could lead to significant gains at the ESS which are not practical at established reactor facilities.

%could run with with similar performance as at a reactorusing the average neutron flux can be built on a reactor as well.

The ideas for intense UCN sources proposed in connection with the WWR reactor \cite{Serebrov2015} or the PIK reactor \cite{Lych2016} cannot be implemented directly in the ESS, due to the design features of this source. \textbf{what features?} Various modifications of these ideas were proposed for ESS at the workshop held in early 2022 as part of the HighNess project \cite{HighNessWorckshop}.
 
An alternative approach is to set up experiments within the converter of a superfluid helium source. This approach makes it possible to use the full accumulated \emph{in-situ} density, which at $220~\text{cm}^{-3}$ for existing prototype sources already exceeds the values that are desirable for next-generation storage experiments. A further advantage is that by eliminating transport losses, one automatically uses the low-energy part of the UCN spectrum which can be most efficiently stored. Extraction-based measurements at any UCN source suffer from the practical compromise that faster UCNs are more easily transported, whereas slower UCNs are more easily stored.

The clear advantages of this approach have been recognized in the past, leading to at least three distinct experimental efforts in this direction \cite{nEDM:2019qgk,Young:2014mxa,Baker:2010zza}. All have confronted significant challenges in the technical implementation of the \emph{in-situ} measurement concept, due to challenges of scale and to the challenge of jointly satisfying the stringent requirements for UCN production and for precision measurements in the same apparatus. It seems clear that to successfully conclude this type of experiment, it is necessary to develop a staged approach in combination with a supporting research and development program. Such an approach has already been proposed to measure the neutron permanent electric dipole moment in connection with the ANNI beamline at the ESS (see section \ref{ANNIsubsubsec:edmn}), and can be similarly envisioned in the context of a dedicated UCN source facility as studied within the HighNESS project.

\emph{In-situ} experiments may provide the most promising avenue to increase the storable density of UCNs with velocities up to 4 m/s, since the required technology for UCN production has already been demonstrated. Given this prerequisite, it becomes possible to significantly improve the accuracy of experiments. In this case, the large gains could be expected in the following cases:
\begin{itemize}
 
  \item [--] improving the accuracy of measuring the neutron lifetime;
  \item [--] precision gravitational neutron spectroscopy;
  \item [--] improving the constraint on the electric dipole moment of the neutron;
  \item [--] experiments to study non-stationary quantum effects \cite{Felber1996}.
\end{itemize}

%One must, however, confront significant technical difficulties . The only such project \cite{Balashov2007}, \cite{CryoEDM_Wiki} has not been brought to a successful implementation.

\subsubsection{Measurements of the neutron lifetime}\label{UCNsubsubsec:taun}
There are several approaches to measuring the neutron lifetime by the UCN storage method. The first group of experiments consists of UCN storage in a trap and measurements of the storage time by following the evolution of the number of UCNs in the trap. In the case of magnetic storage, it is assumed that when the UCN spectrum is formed below the magnetic potential, in the absence of depolarization and inelastic interaction, the storage time is equal to the neutron lifetime. In the case of storage in a material trap, one needs to take into account UCN losses due to the interaction with the walls by measuring the dependence of the storage time on the frequency of collisions of neutrons with the walls and extrapolating this dependence to zero frequency \cite{Kosv1986}. Changing the frequency is achieved either by changing the spectrum of stored neutrons (energy calibration), or by adding additional surfaces to the storage volume, or by changing the volume of the trap (geometric calibration). The losses can be controlled by detecting neutrons escaping the trap via the inelastic scattering channel \cite{Morozov2015}. It is postulated that additional surfaces or surfaces of different traps provide the same loss coefficients. It is possible to calibrate the loss at a fixed collision frequency and change the loss factor, allowing us to get away from this postulate \cite{Alfimenkov1993}.  The second group consists of experiments aimed at detecting neutron decay products in a trap. To date, they have not reached the level of accuracy of the first group \cite{Dzhosyuk2005}, \cite{Picker2005}. 
In experiments with magnetic storage, an accuracy of 0.28~s was achieved \cite{Gonzalez2021}. An increase in statistics in such an experimental setup due to an increase in the phase volume of the experimental setup seems to be unproductive. A significant increase in the strength of constant magnetic fields is technically impossible. An increase of the geometric volume can lead to an increase in systematic effects (an increase in the time for cleaning the spectrum, an increase in depolarization). 
Similarly, in experiments with material traps, the best result to date is 0.7~s \cite{Ser2017}, obtained in a large setup, and a further increase in the geometric dimensions of the trap is hopeless. The broadening of the spectrum of stored neutrons will automatically lead to an increase in the systematics (due to the energy dependence of all characteristic parameters describing the storage and detection of UCNs). It should be noted that in experiments with material traps, it is still tempting to use materials with theoretical low loss factors (such as beryllium and solid oxygen), which have not yet been observed in practice \cite{Alf1992}.
It follows from what has been said that improving the accuracy in any of these approaches requires an increase in the UCN density delivered to an experimental setup. Provided high densities are reached, it is interesting to consider storage of UCNs on the surface of superfluid helium \cite{Alfim2009} and experiments on transformations of the UCN phase volume \cite{Andreev2013}. Such transformations can make it possible to efficiently fill the traps with the soft part of the UCN spectrum.

Speaking about measuring the neutron lifetime in the ESS, one can draw attention to the proposal to determine it from the transformation of the neutron time-of-flight spectrum \cite{Kuz2018}. This proposal has nothing to do with UCN directly, but the observed effect in the proposed experimental design is the larger, the slower the neutrons. It is interesting to consider the possibility of implementing such an approach with UCN (although this will require vertical extraction of neutrons, otherwise it will be difficult to take into account the effect of gravity).

\subsubsection{Gravitational spectroscopy with neutrons}
This section focuses on the control and understanding of a gravitationally interacting elementary quantum system using the techniques of resonance spectroscopy. It offers a way of looking at gravitation at short distances based on quantum interference \cite{Lusch1978}, \cite{Nes2002}, \cite{Abele2010}. The neutron gives access to all parameters related to gravity: distance, mass, curvature, energy momentum tensor, and torsion. Also, the relation between gravitation and quantum theory are probed by investigations of low-energy bound states in the gravitational field. This is possible because the neutron is bound between a flat lying mirror and the raising potential of gravity above, $V=mgz$, where $m$ denotes the neutron mass, $g$ the local gravity, and $z$ the distance above the mirror. Every bound system in quantum mechanics has discrete energy levels. In our case the lowest energy eigenvalues En (n = 1, 2, 3, 4, 5) are 1.4107 peV, 2.4595~peV, 3.3214~peV, 4.0832~peV, and 4.77906~peV. In \ref{fig:GravLev} they are shown together with the corresponding neutron wavefunctions, the well-known mathematical Airy functions as a solution of Airy’s differential equation. Similarly, in the neutron whispering gallery quantum states occur in a binding well formed by the centrifugal potential and a circular boundary \cite{Nes2010}.
\begin{figure}[H]
  \setlength{\unitlength}{1mm}
%\begin{center}
\centering
\hspace{-1.25cm}
  \includegraphics[width=0.61\linewidth, angle=0]{UCN_figure/GravLev.png}
%\end{center}
  %\vspace{-0.75cm}
  \caption{\footnotesize Energy eigenvalues and eigenfunctions of a neutron bound in the gravity potential of the Earth and corresponding frequency equivalents. By oscillating the mirror with a frequency, which correspond to the energy difference between quantum states, transitions are introduced. Shown is a resonant transitions between $|1\rangle \leftrightarrow |6\rangle$ at a frequency of 872.35~Hz. The oscillation frequencies are in the acoustic frequency range.}
  \label{fig:GravLev}
\end{figure}

In 2002 the lowest stationary quantum state of neutrons in the gravitational field was clearly identified \cite{Nes2003}, \cite{Nes2005}, \cite{West2007}. 
The proof of principle triggered new experiments and activity in this direction, namely the setting up of the GRANIT \cite{Granit} and the qBOUNCE \cite{qB} collaboration. 
Spectroscopy is a technique used to assess – in most cases – an unknown quantity of energy by means of a frequency measurement. Basic quantities like atomic masses, particle energies, momenta, and magnetic moments have been determined in this way. The quantum gravitational energy eigenstates can be probed in that way by a coupling to an external resonator. Quantum mechanical transitions with a characteristic energy exchange between the coupling and the energy-levels are observed on resonance. In this Gravity Resonance Spectroscopy (GRS) technique \cite{Jenke2011}, the energy difference between these states has a one-to-one correspondence to the frequency of the modulator, in analogy to the Nuclear Magnetic Resonance technique, where the energy splitting of a magnetic moment in an outer magnetic field is related to the frequency of a radio-frequency field. This is possible due to the feature of the quantum bouncing ball that the levels are not equidistant in energy. The linear gravity potential leads to measured discrete non-equidistant energy eigenstates $|n\rangle$. A combination of any two states can therefore be used, as each transition can be addressed by its unique energy splitting, or, by vibrating the mirror mechanically with the appropriate frequency. In that way GRS is becoming a tool, which combines the virtues of ultracold neutrons (UCNs)
– namely long observation time together with insensitivity to electrostatic and van der Waals interactions
– with spectroscopy, being the method permitting the highest possible sensitivity known.
Highest sensitivity can be reached by applying Ramsey’s method of separated oscillating fields \cite{Abele2010} to GRS. This method will allow a precise measurement of energy differences with a precision similar to the magnetic resonance technique. The statistical sensitivity of the new method at ESS is expected to be around $10^{-21}$~eV. As a consequence, the coupling of residual fluctuations of the magnetic field to the magnetic moment of the neutron must be suppressed to the same level as it is foreseen in a search for an electric-dipole moment. 
The search for generalized gravitational theories is highly topical now. Observational cosmology led to the introduction of the concepts of dark matter (DM) and dark energy (DE). Theoretically, the high-energy behavior and existence of gravitational singularities motivate the search for extensions of Einstein’s General Relativity. At the level of precision, GRS provides constraints on any possible gravity-like interaction. If some as yet undiscovered particles interact with neutrons, this should result in a measurable energy shift of the observed quantum states shown in Fig. \ref{fig:GravLev}  \cite{Jenke2011}, \cite{Jenke2014}, \cite{Cron2018}. 

\subsubsection{Measurements of the neutron's permanent electric dipole moment (EDM)}

Ramsey's method of separated oscillatory fields (see section \ref{ANNIsubsubsec:beamedm}) is the foundational technique used for measuring the neutron EDM, whether using cold neutrons or UCNs. (Another approach has been proposed, exploiting neutron spin-rotation in crystals with very high internal electric fields \cite{Fedorov:2010sj}, but to date has not delivered results at a competitive sensitivity level.) The Ramsey method was initially applied in beam experiments \cite{Smith:1957ht}, until that approach reached systematic limitations due to beam divergence and motional magnetic fields \cite{Dress:1976bq} (see section \ref{ANNIsubsubsec:beamedm} for a discussion of how these effects might be mitigated in modern experiments at the ESS). At that point, UCNs offered a viable way forward both by mitigating these particular systematic effects and by opening the door to much longer observation times \cite{Altarev:1980rgh}. Since that time, all further advances in accuracy for measurements of the neutron EDM have been based on storage experiments with UCNs in a measurement volume separate from the UCN source.

A key subsequent development was the concept of ``comagnetometry" \cite{Lamoreaux:1989gy}, in which an atomic species with a similar sensitivity to magnetic fields -- but whose EDM is expected, or has been measured, to be small -- co-occupies the measurement volume with the UCNs. This enables a simultaneous differential measurement, in which all effects seen by the comagnetometer are subtracted in common-mode under the assumption that only the UCNs are sensitive to CP-violation through an EDM. This approach greatly extends the sensitivity of such measurements, at the expense of experimental complexity and certain limitations on the experimental conditions (e.g., electric field strength) that may be required in order for the comagnetometer to function. One may note, however, that the leading systematic errors for the most recent neutron EDM measurement were associated with the comagnetometer correction \cite{Abel:2020gbr}; new experimental proposals are increasingly favoring tight control of experimental conditions rather than contending with the increasing challenges of comagnetometry at higher levels of sensitivity.% This places much more stringent demands on the stability and monitoring of experimental conditions, but removes the need to correct for increasingly nuanced effects due to the comagnetometer alone, as new levels of sensitivity are approached.

A further conceptual advance, now universally adopted in the present generation of neutron EDM experiments, was to perform two measurements simultaneously with a common magnetic field and oppositely-directed electric fields \cite{Altarev:1996xs}. This effectively removes any drift within the pairs of measurements that must be combined in order to determine the EDM. When in addition a comagnetometer is present in both cells, one can also remove in this way the leading effects connected with magnetic field gradients. A generalization of this concept to many cells has been proposed by Serebrov \cite{serebrov2007multi}, which in suitably stable conditions would permit controlling this type of systematic effects to arbitrary order. This concept is also central to the implementation of the EDM$^n$ project at the ESS (see section \ref{ANNIsubsubsec:edmn}).

While improved statistics may be the main route to long-term improvements in measurements of the neutron EDM, one should also note that gains can still be had from increasing the observation time and electric field strength -- parameters for which the scaling is actually more favorable, see equation \ref{ANNIsubsubsec:edmeqn}. Due to numerous constraints on the holding cell geometry and material composition, and unlike experiments measuring the neutron lifetime, the longest achieved holding times for neutron EDM measurements are on the order of $200~\text{s}$ -- significantly shorter than the ultimate limit of $880~\text{s}$. Recent demonstrations of long UCN storage lifetimes in small bottles \cite{neulinger-thesis}, with material coatings intended for EDM applications and using soft UCN spectra extracted from a superfluid-helium source, have given rise to hopes that the storage time in particular may provide a route toward improvements in the next generation of experiments. The electric field strength is typically limited to the order of $2~\text{MV/m}$ (or less, in the presence of a comagnetometer) by the surface conductivity of the insulating ring which forms one wall of a UCN storage cell. However, recent advances in cryogenic technology developed for an \emph{in-situ} neutron EDM measurement by the American collaboration nEDM@SNS have indicated that much higher fields, on the order of $10~\text{MV/m}$ can be sustained when the cell is filled with superfluid helium \cite{Phan:2020nhz}. This brings the electric field strength into the same range as for the BeamEDM experiment (see section \ref{ANNIsubsubsec:beamedm}).


\subsection{Prospects for the use of VCN}
Nowadays, very cold neutrons (energies $<10^{-4}$ eV) are practically not used in neutron physics. Despite the periodic discussion of the advantages of their use \cite{ANL2005}, \cite{ORNL2016} \cite{ESS2022}, the development of this field is hampered both by the lack of intense sources of these neutrons (the only available source of VCN is in ILL \cite{pf2_VCN}) and by the need to adapt experimental setups and existing techniques. At the same time, overcoming these difficulties promises to expand the field of using neutrons both for solving problems in particle physics and in the field of neutron scattering. In recent years, efficient reflectors of VCN are developed  \cite{Nes2008_ref_VCN}, \cite{Lych2009}, \cite{Lych2009_store}, \cite{Nes2010_ApND}, \cite{Cubitt2010}, \cite{Kry2011}, \cite{Lych2013}, \cite{Art2006}, \cite{Shab2012}, \cite{Ign2014}, \cite{Art2016}, \cite{Tesh2019}, \cite{Ersez2018}, \cite{Gran2020}, \cite{Jama2020}, \cite{Gram2020}, \cite{Jama2020_G4}. These reflectors can help significantly increase the VCN flux, available in experiments. Optimization of moderators using the reflectors for specific neutron sources is a matter for the near future.
Here we will only briefly list the ideas of using VCN that are known to us:
\begin{itemize}
    \item Search for neutron-antineutron oscillations \cite{VCN_n_nbar}. The idea of an experiment with cold neutrons was discussed above in Section 6. The sensitivity of the experiment is proportional to the product of the observation time of oscillation and the square root of the neutron flux. The switch to slower neutrons with the same experimental setup does not  give a gain at first glance. The observation time is inversely proportional to the neutron longitudinal velocity, and the neutron flux in the neutron guide is proportional to the square of the velocity (under the natural assumption that the neutron phase density in the source is constant). However, the use of the above-mentioned reflectors can in principle make it possible to significantly increase the phase density of the VCN \cite{Nes2022_VCN}.
    \item Search for the electric dipole moment (EDM) of the neutron \cite{Piegsa2013}. As in the case of neutron-antineutron oscillations (considered just now), in the experiment on the search for the neutron EDM discussed in Section 4.3.1, a gain is possible when switching to slower neutrons. In addition, the use of slower neutrons should reduce the relativistic corrections.
    \item Search for additional types of interactions \cite{Snow2022} by studying the angular distribution of neutrons scattered by atoms of noble gas.
    \item The sensitivity of the interferometers discussed in Section 5 depends on both the intensity and the parameters of the optical system. Slow neutrons have a higher refractive index and, accordingly, the requirements for the optical system become not so strong, and the optical effects are more pronounced. Interferometers can be used for precision measurements of the coherent length of neutron scattering by nuclei, search for new types of interactions.
    \item The use of VCN in a beam experiment to measure the neutron lifetime \cite{Nico2013} will increase the observation time, and proportionally to it the detected signal from neutron decay.
    \item Increasing the sensitivity of commonly used neutron scattering techniques such as spin echo \cite{Mezei1972}, \cite{Hino2003} (by increasing the observation/interaction time) and reflectometry (by expanding the dynamic range of the setup) \cite{Baes2011}.
    \item Use of tomography with VCN for solving specific problems \cite{Maru2005}.
\end{itemize}



==> glossary.tex <==
\makeglossaries

\newglossaryentry{latex}
{
        name=latex,
        description={Is a mark up language specially suited for 
scientific documents}
}

\newglossaryentry{maths}
{
        name=mathematics,
        description={Mathematics is what mathematicians do}
}

\newglossaryentry{formula}
{
        name=formula,
        description={A mathematical expression}
}

\newacronym{gcd}{GCD}{Greatest Common Divisor}

\newacronym{lcm}{LCM}{Least Common Multiple}

==> interf.tex <==
\section{Neutron interferometry at the ESS}
\label{sec:neutroninterferometry}

%{\em Authors: Hartmut Abele, Stephan Sponar, Yuji Hasegawa, Hartmut Lemmel and Michael Jentschel, 1.5 pages}
\subsection{Introduction }
Interferometer experiments with neutrons date back to 1960ies, where progress in semiconductor technology made it possible to produce monolithic perfect crystal silicon ingots, with a diameter of several inches, from which a single-crystal interferometer (based on knowledge for X-ray interferometry) can be cut out. In 1974 such an interferometer was illuminated with thermal neutrons, which resulted in the first observed interference fringes by Rauch, Treimer and Bonse at the TRIGA research reactor at the Atominstitut - TU Wien, in Vienna, Austria. In a neutron interferometer, a beam of neutrons is split by amplitude division, and superposed coherently after passing through different regions of space \cite{Rauch1974,Rauch2000,Sponar:2020gfr}. During these macroscopic spatial separation, the neutron’s wavefunction can be modified in phase and amplitude in various ways. Neutron interferometry enabled several text-book experiments, such as demonstrations of $4\pi$ spinor symmetry of spin-1/2 particles, spin superposition, gravitationally induced phase and topological phase effect, as well as studies of characteristics of intra-partite entanglement, i.e., entanglements between different degrees of freedom \cite{Hasegawa2003} or studies of anti-commuting properties of Pauli spin matrices. In more recent times weak values and related quantum paradox (e.g.\ Quantum Cheshire Cat) have been studied in neutron interferometric experiments.
\subsection{Description/method}
In the interferometer (see Figure~\ref{ANNIfig:Interferometry1} for an illustration and Figure~\ref{ANNIfig:Interferometry2} for photos), neutrons exhibit self-interference, since at any given instant at most a single neutron propagates through the interferometer. The interferometer is geometrically analogous to the well-known Mach-Zehnder interferometer in photonics. Neutrons are affected by all four fundamental interactions, which are used in realising neutron optical components, including nuclear (weak and strong), gravitational  and magnetic  phase shifts. By rotating the phase shifter plate by an angle $\eta$, the phase shift $\chi$ can be tuned systematically, due to the change of the relative optical path length in path I and path II. After rotation of the entire interferometer by an angle $\alpha$ around the incident beam direction by employing a tilting stage the neutron’s split wave packets travel at different heights, and therefore at different gravitational potentials. The neutron couples to magnetic fields via its permanent magnetic dipole moment $\mu$, where static as well as time-dependent magnetic fields are used to realise arbitrary spinor rotations due to the Larmor precession of the neutron’s polarisation vector. With time-dependent magnetic fields not only the neutron’s spin but also its total energy can be manipulated due to photon absorption or emission.
\subsection{Sensitivity (in function of ESS power)}
The sensitivity of interferometers are related to the neutron flux, and depending on the scientific question, the loop of the neutron’s wavepacket’s motion around the interferometer, or the length of separation between the splitting crystals. At ESS new concepts of interferometers can be explored. Most promising are split crystal interferometers.
\subsection{Discussion with respect to theories and current and projected experiments elsewhere}
Due to the small polarisability of neutrons compared to atoms or molecules, neutron interferometry is considered complementary to interferometer methods with atoms. In focus are tests of fundamental concepts of quantum mechanics or basic symmetries. Examples are e.g.\ investigations of the completeness of quantum errors, weak values and commutation relation, entropic noise-disturbance uncertainty relations, searches for dark energy and dark matter particles etc. The unique design of the ESS, with a proton pulse of 2.86~ms and a repetition rate of 14 Hz, opens the door for new experimental techniques in the field of neutron interferometry, such as studies of quantum dynamics, or various interactions on short time scales.
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{AnniFigs/Interferometry1.png}
    \caption{Illustration of neutron interferometry 1.}
    \label{ANNIfig:Interferometry1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{AnniFigs/Interferometry2.png}
    \caption{Illustration of neutron interferometry 2.}
    \label{ANNIfig:Interferometry2}
\end{figure}



==> nnbar-draft.tex <==
  Of all the empirically observed conservation laws, the conservation of baryon number is arguably the most fragile. Should baryon number violation (BNV) not be a feature of Nature, the Standard Model would be falsified~\cite{Klinkhamer:1984di} and the dynamic generation of the observed matter-antimatter symmetry would not be possible~\cite{Sakharov:1967dj} . It is perhaps most appropriate to discuss not {\it whether} baryon number violated but {\it in which channels} baryon number is violated.   The HIBEAM/NNBAR program\footnote{The High Intensity Baryon Extraction And Measurement (HIBEAM) phase would take place at a fundamental physics beamline and would be followed by the NNBAR phase using the Large Beam Port.} takes advantage of the unique opportunity provided by the world's brightest neutron source, the ESS, for a multi-stage and long-term series of experiments of increasing sensitivity to search for BNV via the conversion of neutrons to anti-neutrons and/or sterile neutrons. The program encompasses $\Delta B=1,2$ processes and will achieve a sensitivity improvement in neutron conversions by three orders of magnitude compared with previous searches~\cite{Bressi:1989zd,Bressi:1990zx,Fidecaro:1985c m,BaldoCeolin:1994jz}.  
  
  Like the photon (axions) and the neutrino (sterile neutrinos), the neutron is an ideal probe for mixing processes beyond the SM~\cite{Nussinov:2001rb,Dvali:1999g,Barbier:2004ez,Dutta:2005af,Calibbi:2016ukt,Berezhiani:2015uya,Dev:2015uca,Allahverdi:2017edd,Dvali:2009ne}.  It is electrically neutral and quasi-stable, can be copiously produced, and the observation of neutron mixing would address open questions in modern physics.  As mentioned above and described in section~\ref{sec:theorynnbar}, the program BNV-violating neutron conversions into anti-neutrons and/or sterile neutrons addresses both the matter-antimatter asymmetry and could point to the existence of a hidden sector of particles, and thus shed light on dark matter\cite{Berezhiani:2003xm,Berezhiani:2005ek}.
  
  
  

==> theory_old.tex <==
%ages)
%        \item oscillations (among the SM three flavors and to additional exotic states), CP violation in the leptonic sector, non-standard neutrino interactions with matter: Tommy Ohlsson/Zurab (1.5 pages)
%   \end{enumerate}
%\end{enumerate}

%\subsection{General introduction}

%Put the problems first(Valery)
%The main goals of fundamental physics are testing the present theory, the Standard Model (SM), and looking for phenomena beyond it. 
The Standard Model (SM) of particle physics \cite{Glashow:1961tr,Weinberg:1967tq,Salam:1968rm} describes a very large body of experimental results but it has a number of shortcomings and issues to which it does not have a good answer. One of the shortcomings is the large number of free parameters, especially in the so-called flavour sector where the pattern of quark and lepton masses and mixing is simply put in by hand, see e.g.~\cite{Gori:2019ybw}. A related issue is the origin of neutrino masses and mixing, see Section~\ref{sec:theoryneutrinooscillations} and e.g.~\cite{Fantini:2018itu}. These issues could be described as "close to the SM" questions. There is also the QCD-theta parameter leading to CP-violation in the purely strong sector which is unnaturally small.%\footnote{See however references \cite{Nakamura:2019ind,Nakamura:2021meh,Ai:2020ptm,Ai:2022htq} which using different methods suggest that CP is conserved in strong interactions.}

The next class of issues concerns those related to the universe and the question of why matter exists. We know that a large part of the energy density of the universe is not normal matter, i.e. it cannot be explained by particles and fields present in the SM. This consists of two types, dark matter and dark energy. The former is most likely due to some particles only interacting weakly with normal matter while the nature of the latter is fully unclear, but compatible with a simple cosmological constant, see e.g. \cite{DeSimone:2019lmz}. The question of why matter and anti-matter are not created in equal amounts in the early universe also falls into this class.

The third class of issues is that where we have little experimental clue as to what to expect. These include quantum gravity, searching for violations of Lorentz and CPT symmetries and in general searching for processes and phenomena not present in the SM. 

The last class is related to studying effects of the strong interaction, especially in ways that help to answer some of the experimental uncertainties appearing for the others, but also interesting in their own right.

The resolution of the above-mentioned SM shortcomings likely requires new degrees of freedom and 
new dynamics. This strongly motivates a broad search for new physics, by either performing precision measurements of SM-allowed phenomena or by searching for phenomena that are `rare' or forbidden, because they violate approximate or exact symmetries of the SM. One should of course also be on the look-out for surprises, completely unexpected new results.

In broad brush terms one can expect that new physics has escaped detection so far because the new particles are either very heavy or very weakly coupled. Traditionally, there are two routes to search for new physics in laboratory experiments:  one is to increase the  energy of particle accelerators so as to try to  directly produce new particles -- this is known as the ``energy frontier". 
The other approach is to  perform very precise and sensitive measurements in low invariant mass systems, which allows one to indirectly access the virtual exchange of heavy degrees of freedom or directly excite light and weakly coupled particles  -- this is known as the ``precision frontier''.  
This second route  requires using ultra-sensitive detectors and/or powerful particle accelerators to generate large fluxes of particles such as neutrinos, muons, mesons, neutrons, etc. --  hence sometimes the name  ``intensity frontier''. In this language, the ESS is an intensity frontier facility. 

We emphasize that both  energy and precision/intensity frontiers are needed to infer structure, symmetries, and parameters of the underlying new physics. For example, while high-energy colliders are the most powerful probe of new particles associated to the electroweak symmetry breaking mechanism,  precision frontier experiments typically provide the strongest probes of lepton ($L$) and baryon ($B$) number violation, CP violation, flavor violation in the quark and lepton sectors, charged- and neutral-current weak interactions, neutrino properties, and dark sectors.

In the context of the intensity frontier, the ESS will provide a number of exciting opportunities, 
due to the high neutron and neutrino fluxes. First, precision measurements of neutron decay will probe non-standard interactions in the charged-current sector and help to determine the mixing element $V_{ud}$ precisely, Section~\ref{sec:theorybetadecay}. Second,  measurements of the neutron electric-dipole moment, Section~\ref{sec:theoryedm}, provide the most sensitive probe for CP-violation beyond the SM, as well as stringently bounding the QCD-theta parameter. Baryon number violation has been strongly probed in proton decay but alternatives that do not contribute to this exist and can be probed via neutron oscillations to anti-neutrons or sterile neutrons (see  Section~\ref{sec:theorynnbar}). Both of these will contribute to the understanding of net baryon number generation in the universe. Another strength of the ESS will be the searches for extra fundamental interactions and other phenomena discussed in Section~\ref{sec:theoryextra}. 
The nucleon-nucleon weak interaction is expected to have a number of nontrivial features and possible measurements are discussed in Section~\ref{sec:theoryhpv}.
Moreover, neutrino oscillation measurements will be sensitive to CP violation in the lepton sector 
and non-standard neutrino interactions with matter (see Section~\ref{sec:theoryneutrinooscillations}).
Precise measurements of coherent neutrino-nucleus scattering will test neutrino couplings to quarks and help in determining reaction rates for dark matter experiments, as outlined in Section~\ref{sec:theoryneutrinoscattering}.

In the theory part of this review we have chosen to discuss the physics relevance for the different experimental activities mainly in terms of specific models when we address sensitivities to physics beyond the Standard Model. An alternative way to do this is to use effective field theory (EFT) methods, see e.g. \cite{Penco:2020kvy} for a general introduction. There are several reasons why we did not choose this method for comparison with e.g. direct searches:
\begin{itemize}
\item Each experiment typically comes with its own relevant EFT or at least its own relevant combination of coefficients in the EFT. Examples are Chiral perturbation theory for a lot of hadron physics, chiral (nuclear) effective theory for nuclear effects, Standard Model Effective Field Theory (SMEFT) and Higgs Effective Field Theory (HEFT), see e.g. \cite{Brivio:2017vri}, for LHC physics, Low-Energy effective field theory below the electroweak scale \cite{Jenkins:2017jig} for
%and the operators describing the different decay formfactors in 
neutron beta decay.
\item Comparison with direct searches for mediator particles at the LHC and other high energy colliders are typically model dependent.
\end{itemize}
On the other hand, for low-energy experiments as ESS experiments typically qualify, putting the results in terms of the relevant EFT coefficients makes comparison with models easier. It also shows the importance of doing complete measurements.

Next, we discuss in greater details the opportunities discussed above.


\subsection{Neutrons}
\label{sec:theoryneutrons}

\subsubsection{Precision measurements in neutron beta decay}
\label{sec:theorybetadecay}

Beta decay has played a crucial role in the history of particle physics (neutrino hypothesis, parity violation, V-A theory, ...)~\cite{Pauli:1930pc,Fermi:1934hr,Cowan:1956rrn,Lee:1956qn,Wu:1957my,Weinberg:2009zz}. Neutron beta decay is particularly interesting for several reasons. First, it is the simplest one from a theoretical point of view (other than the pion beta decay, which has a branching ratio of $10^{-8}$), since nuclear effects are absent in this case. Second, it is sensitive to a wide variety of interactions, since both Fermi and Gamow-Teller matrix elements are non-zero. Third, significant progress is taking place on the experimental side with the arrival of powerful (ultra)cold neutron sources and new detection techniques~\cite{Abele:2008zz,Dubbers:2011ns,Baessler:2014gia,Dubbers:2021wqv}.

During the last decades there were significant tensions between some of the measurements~\cite{Abele:2008zz,Dubbers:2011ns,Wietfeldt:2011suo}, which inspired interesting theory developments that illustrate the broad discovery potential of neutron beta decay measurements, see {e.g.} Refs.~\cite{Fornal:2018eol,Berezhiani:2018eds}. Although the internal consistency of the data has greatly improved with the arrival of more precise measurements and the revision of some of the older ones, some tension remains, affecting quantities as important as the neutron lifetime~\cite{Falkowski:2020pma,Zyla:2020zbs}. It would be highly desirable to further clarify the situation. 

The exquisite theory and experimental precision achievable in several observables makes neutron beta decay sensitive to small effects generated by a wide variety of new phenomena~\cite{Herczeg:2001vk,Cirigliano:2013xha,Vos:2015eba,Gonzalez-Alonso:2018omy}. These measurements can probe heavy new particles, which can be too massive to be produced at the LHC~\cite{Bhattacharya:2011qm}. %,Cirigliano:2013xha}. 
Such particles could play a crucial role in the generation of the matter-antimatter asymmetry or the electroweak symmetry breaking mechanism. 
Likewise, beta decay measurements are sensitive to the effects of new light particles with very small couplings to the known fields, opening an interesting connection with dark matter searches.%~\cite{}.

The physics reach of neutron beta decay goes beyond such searches of new phenomena. It gives us access to the mixing matrix element $V_{ud}$, one of the fundamental parameters of the electroweak sector in the SM. 
Recent studies have increased the accuracy of the radiative corrections to neutron beta decay, while revealing new uncertainty sources in nuclear decays, strengthening the case of the former to extract $V_{ud}$~\cite{Seng:2018yzq,Seng:2018qru,Gorchtein:2018fxl}. 
Testing the unitarity of the CKM quark mixing matrix, whose $(1,1)$ element is $V_{ud}$, represents a crucial check of theory~\cite{Gonzalez-Alonso:2018omy}. It should be clarified whether recent tensions in this test are unaccounted SM effects or hints of new phenomena~\cite{Grossman:2019bzp,Coutinho:2019aiy,Cirigliano:2021yto}. 
%
%
%
%
Neutron decay is also of the highest importance for the study of strong interactions thanks to the precise extraction of the axial nucleon charge $g_A$ and the study of the above-mentioned radiative corrections. The comparison with QCD predictions is a challenging test~\cite{Chang:2018uxx,Gupta:2018qil} that is sensitive to nonstandard effects~\cite{Gonzalez-Alonso:2018omy}. %right-handed currents~\cite{Gonzalez-Alonso:2016etj}. 
Finally, neutron decay measurements are relevant as well for nuclear physics, astrophysics and cosmology, where $g_A$ and $V_{ud}$ play a crucial role~\cite{Abele:2008zz,Dubbers:2011ns,Suhonen:2017krv}. 

As explained in %Sections~\ref{ANNIsubsec:Intro} and~\ref{ANNIsubsec:ndecay}
Sections~\ref{ANNIsubsec:ndecay} and~\ref{UCNsubsec:taun}, the ESS offers a unique possibility to improve our knowledge of fundamental properties of the neutron beta decay. Significant improvements are expected both on the SM parameters and the BSM searches, with the many and varied implications that were mentioned above.

%[TO BE CONTINUED]
%{\bf Expected improvement at ESS:}  ${\cal O}(10)$ improvement in $A$ and $\tau_n^{bottle}$. For beam measurements we can expect $\sim 1 s$ with great control of the systematic errors that should help clarifying the situation. Before ESS, we should have a new beam measurement at NIST.
%Possible experimental improvements at the ESS are discussed in section~\ref{ANNIsubsec:ndecay}.



\subsubsection{Searches for a non-zero neutron electric dipole moment}
\label{sec:theoryedm}



Permanent electric dipole moments (EDMs)  of non-degenerate quantum systems,  such as the neutron, 
would signal  the breakdown of time-reversal (T) and parity (P) invariance, 
or equivalently (due to the CPT theorem) of CP invariance,   where C is the charge conjugation operation that exchanges particles and antiparticles.
Given the un-observably small contribution to EDMs induced by the SM weak interactions, the current null EDM results 
and prospective sensitivities have far-reaching implications for  fundamental interactions and cosmology, as briefly summarized below 
(for more extended discussions see Refs.~\cite{Pospelov:2005pr,Engel:2013lsa,Chupp:2017rkp}).

First, the existing upper limits on neutron EDM ($\vert d_n\vert < 1.8 \times 10^{-26}$ $e$~cm at 90\% CL\cite{Abel:2020gbr})
imply that CP-violating effects in the SM strong interaction are  extremely  small 
($|\theta_{\rm QCD} |< 10^{-10}$).  This is already pointing to something very deep and historically, even before the bound 
became so stringent,  has led to the idea of a new  broken symmetry whose Goldstone boson -- the axion -- is  a viable candidate for 
the dark matter in the universe~\cite{Peccei:1977hh,Weinberg:1977ma,Wilczek:1977pj}.
Second, the current null EDM results severely constrain extensions of the SM  that include CP-violation at the TeV scale, 
and probe very strongly the CP properties of the  recently discovered Higgs boson and possible extended Higgs sectors. 
Finally, EDM searches shed light on the origin of the matter-antimatter asymmetry of the universe, 
which cannot be explained  within the SM and requires the presence of new CP violation, according to Sakharov's conditions~\cite{Sakharov:1967dj}.


To pin down the nature of new sources of CP violation,  multiple EDM searches are needed,  as EDMs of different particles species posses different sensitivity to possible contributions from quark EDMs and color-EDM,  purely gluonic CP-violating interactions, and CP-violation in the lepton sector~\cite{Chupp:2017rkp}. 
In this context the neutron stands out as the theoretically cleanest hadronic system.  In fact,  there are good prospects  to reduce the uncertainty associated with non-perturbative QCD effects in the near future with lattice QCD~\cite{Bhattacharya:2015esa,Abramczyk:2017oxr,Kim:2021qae,Dragos:2019oxn}, 
thus enhancing the model-diagnosing power of neutron EDM searches (both in case of positive and null signal).  

The gap between the existing upper limits on neutron EDM ($\vert d_n\vert < 1.8 \times 10^{-26}$ $e$~cm at 90\% CL\cite{Abel:2020gbr}) 
and the Standard Model expectation due to the Kobayashi-Maskawa phase 
($\vert d_n\vert \sim 10^{-32}$ $e$~cm~\cite{Seng:2014lea}) provides a compelling discovery window spanning six orders of magnitude. Current and next generation searches will have sensitivities a few orders of magnitude 
below the current limits. 
The major scientific merits of a one to three order of magnitude improvement in the neutron EDM sensitivity [i.e. $\vert d_n\vert \sim (10^{-29} - 10^{-27}) e~{\rm cm}$]  are:

(i) Sensitivity to very high scale new physics, possibly inaccessible at current colliders.   Existing null EDM results  already imply a lower bound of several TeV on the mass scale $M$ associated with new CP violation, based on general effective theory considerations. These model-independent considerations  are borne out in detailed studies of explicit models, such as the minimal supersymmetric standard model~\cite{Li:2010ax}  and the so-called split-supersymmetry 
scenarios~\cite{Giudice:2004tc,ArkaniHamed:2004yi,Altmannshofer:2013lfa,McKeen:2013dma,Bhattacharya:2015esa}, where the future sensitivity reaches up to hundreds of TeV. 


(ii) Unmatched sensitivity to  CP-violating interactions of the Higgs boson~\cite{McKeen:2012av,Brod:2013cka,
Chien:2015xha} and of extended Higgs sectors~\cite{Inoue:2014nva}.
 This makes the neutron EDM a key  tool in  characterizing  the  properties  of the Higgs boson discovered at the LHC in 2012 and baryogenesis, see e.g. \cite{Fuchs:2020uoc}.

(iii)  The possibility to probe mechanisms  for the generation of the baryon asymmetry of the universe. 
 With the observation of the Higgs boson, it is particularly timely to ask whether the baryon asymmetry was produced during the electroweak symmetry-breaking era that occurred roughly 10 picoseconds after the Big Bang,  involving new particles with masses around or below the TeV scale (see Ref.~\cite{Morrissey:2012db} for a review). 
 EDM searches provide a particularly powerful probe of the associated CP violation, given their sensitivity to mass scales M in the multi-TeV region.   In many scenarios 
 (with some  exceptions~\cite{Li:2008ez})   successful baryogenesis leads to strict lower bounds on the neutron and electron EDMs,  only a factor of 2 -- 3 below the current experimental limits~\cite{Cirigliano:2009yd,Morrissey:2012db}.
 The new generation of neutron EDM searches will provide very stringent tests of the  origin of matter in baryogenesis mechanisms operating near the electroweak scale. 
 
 Experimental prospects for neutron EDM searches at ESS are discussed in Sections~\ref{ANNIsubsec:EDM} and \ref{sec:UCNedm}.


%[NEED TO ADD MORE REFERENCES; add general comments on other probes of CP violation, with and without flavor change]



\subsubsection{Neutron oscillations to anti-neutrons or to sterile neutrons}
\label{sec:theorynnbar}

The possibility of neutron--antineutron ($n-\bar{n}$) oscillation was put forward  
 in Refs. \cite{Kuzmin:1970nx,Glashow:1979nm,Mohapatra:1980qe}, 
followed by a number of papers studying different aspects 
of this phenomenon and its model realizations \cite{Mohapatra:1980de,Kuo:1980ew,Cowsik:1980np,Chetyrkin:1980ta,Barbieri:1981yr,Caswell:1982qs,Rao:1982gt,Rao:1983sd}. 
The neutron--antineutron oscillation violating baryon number $B$ by two units can have an intimate 
connection with the possibility of neutrino Majorana masses which violate lepton number $L$ 
by two units (and both violate $B-L$). 
In particular this connection can naturally emerge e.g. in a left-right symmetric model 
or its $SO(10)$ extensions,
in which $U(1)_{B-L}$ is a local symmetry and it has to be spontaneously broken at some scale 
\cite{Mohapatra:1980qe}.  

In the SM the neutron can have only Dirac mass while the neutrinos remain massless. 
But in the context of BSM theories the neutrino Majorana masses can be induced via 
the effective $\Delta L=2$ operators $C_{L=2} (\ell \phi)^2 $ of dimension 4 
involving two lepton doublets $\ell$ \cite{Weinberg:1979sa},  
where $\phi$ stands for the Higgs doublet of the SM. 
Then the neutrino mass range $m_\nu \sim 0.1$~eV implies the Wilson coefficient 
$C_{L=2} = M_{L=2}^{-1} \sim (10^{14}~\text{GeV})^{-1}$
pointing to a lepton number breaking scale close to the GUT scale.  
%at which operators $(1/M_G^2) qqq\ell$,  violating $B$ and $L$ but conserving $B-L$, 
% are induced in the grand unified theories.  
As for the neutron Majorana mass term $\epsilon_{n\bar{n}} n^T C n +\mathrm{h.c.}$ 
responsible for $n-\bar{n}$ mixing, 
it can be originated from the six-quark (dimension 9) operators $C_{B=2} (udd)^2$ 
involving $u$ and $d$ quarks  in combinations with different Lorentz and color structures 
\cite{Caswell:1982qs,Rao:1982gt,Rao:1983sd}.  
However, the determination of the effective scales $M_{L=2}$ and $M_{B=2}=C_{B=2}^{1/5}$ 
 is a model dependent issue, and even in the GUT context their values can be quite different. 
Namely,  $\Delta B=2$ operators induce $n-\bar{n}$ mixing with 
$\epsilon_{n\bar{n}} = \kappa(1~{\rm PeV}/M_{B=2})^5 \times 3 \cdot 10^{-25}$~eV, 
 $\kappa=O(1)$ being the operator dependent constant in the evaluation of the matrix element 
$\langle 0\vert udd \vert n\rangle$. The value of $\kappa$ is calculated by lattice QCD and models see \cite{Rinaldi:2019thf,Bijnens:2017xrz}. Indirect limits from decay of nuclei are affected by large uncertainties~\cite{Oosterhof:2019dlo,Haidenbauer:2019fyd}.
 The direct experimental bound on the $n-n'$ oscillation time 
$\tau_{n\bar{n}} = \epsilon_{n\bar{n}}^{-1} > 8.6\times 10^7$~s \cite{BaldoCeolin:1994jz}, 
implies  the upper limit $\epsilon_{n\bar{n}} < 7.7 \times 10^{-24}$~eV. 
Somewhat stronger but indirect bounds follow from the nuclear stability, namely from oxygen 
$\epsilon_{n\bar{n}} < 2.5 \times 10^{-24}$~eV,  so that present limits point  
to the effective scale of around $M_{n\bar{n}} > 0.5$~PeV. 
(For a summary of the present experimental situation, see the reviews 
\cite{Phillips:2014fgb,Babu:2013yww}.) 
Therefore, the experimental search of $n-\bar{n}$ oscillation can be meaningful if the scale $M_{6q}$ 
is below around 10~PeV. On the other hand, its discovery would be a clear evidence of $B$-violation by two units,  
and would have a great impact for our understanding of the origin of the baryon asymmetry in the universe. 
 
The last two decades showed a renaissance of the interest for new physics related to $n-\bar{n}$ mixing,  and generally for $\Delta B =2$ processes and their role in the early universe. 
In particular, new theoretical schemes involving new particle states mediating the effective six-quark 
operator were proposed and their implications for the LHC searches and for primordial 
baryogenesis were discussed 
\cite{Berezhiani:2005hv,Dutta:2005af,Babu:2006xc,Babu:2008rq,Babu:2013yca,Dev:2015uca,McKeen:2015cuz,Calibbi:2016ukt,Allahverdi:2017edd,Grojean:2018fus,Bringmann:2018sbs}.  
Mechanisms of $n-\bar{n}$ mixing were discussed also in the context of the theories with extra 
dimensions \cite{Dvali:1999gf,Nussinov:2001rb,Girmohanta:2019fsx,Girmohanta:2020qfd}. 
Different theoretical aspects of $n-\bar{n}$ oscillation were also discussed regarding the role of discrete  C, P, T symmetries
\cite{Berezhiani:2018xsx,Berezhiani:2018pcp,Tureanu:2018phm,Fujikawa:2020gsa},
as well as the possibility of the very low scale spontaneous $B-L$ violation by two units and its apparent effects \cite{Berezhiani:2015afa,Addazi:2016rgo,Babu:2016rwa}. 


Another stream of research that emerged in the last two decades 
is related to a possible connection between the neutron and dark matter (DM),  
in particular in the context of the scenarios where DM is represented  by a hidden gauge sector.  
The simplest and most economic example is related to mirror particles \cite{Lee:1956qn,Kobzarev:1966qya}. 
Namely, a dark sector represented by a mirror 
SM$'$ replica of the SM,  which means that all observed particles: the electron $e$, 
proton $p$, neutron $n$ etc. must have their dark mirror twins $e'$, $p'$, $n'$ etc. which are 
sterile to our SM interactions but self-interact via the SM$'$ gauge bosons 
(for reviews see \cite{Berezhiani:2003xm,Berezhiani:2005ek}). 
Mirror matter is a viable candidate for DM with specific cosmological implications
 if, after inflation, mirror sector was reheated at lower  temperatures than the ordinary world  
\cite{Hodges:1993yb,Berezhiani:1995am,Berezhiani:1996sz,Berezhiani:2000gw,Berezhiani:2003wj}. 
During cosmological evolution, as for ordinary matter, 
the mirror nuclei and atoms, as well as stellar objects, which are dark for an ordinary observer, should form. 

Besides gravity, there can exist some feeble interactions between  particles of two sectors 
induced e.g. by kinetic mixing of the ordinary and mirror photons 
\cite{Holdom:1985ag,Glashow:1985ud} and/or  
by gauge bosons of common flavor symmetry \cite{Berezhiani:1996ii,Belfatto:2018cfo}. 
These interactions can provide a portal for the direct DM detection  
\cite{Foot:2008nw,Addazi:2015cua,Cerulli:2017jzz} and induce the mixing phenomena 
between the neutral particles of two sectors as pions and Kaons. 
Ordinary and mirror sectors can be connected also by a common axion 
\cite{Berezhiani:2000gh}. 
However, most interesting are the interactions which violate baryon and lepton numbers 
of both sectors. From the one hand, such interactions can provide a 
co-genesis mechanisms of baryon asymmetries both in ordinary and mirror worlds 
which can naturally explain the relation between the baryon and DM fractions 
in the universe \cite{Bento:2001rc,Berezhiani:2008zza,Berezhiani:2018zvs}. 
On the other hand, they can induce the mixing of the neutrinos and the neutron 
with their dark mirror partners, exactly or closely degenerate in mass. 

Namely, dimension 5 operators $C_{L=1} (\ell \phi)(\ell \phi)' $, 
which violate lepton numbers $L$ and $L'$ of both sectors by one unit,
induce active-sterile $\nu-\nu'$ mixings  
which makes  mirror neutrinos natural candidates for sterile neutrinos 
\cite{Akhmedov:1992hh,Foot:1995pa,Berezhiani:1995yi}. 

Analogously, mass mixing between the ordinary $n$ and sterile mirror $n'$ neutrons, 
$\epsilon_{nn'} n^TCn' +\text{h.c.}$, can be induced  
by dimension 9 operators $C_{B=1} (udd)(u'd'd')$ 
involving ordinary $u,d$ and mirror $u'd'$ quarks 
which violate both $B$ and $B'$ but conserve the combination $B-B'$ \cite{Berezhiani:2005hv}. 
As opposed to $n-\bar{n}$ mixing, the nuclear stability limits give no restriction 
on $n-n'$ mixing since $n\to n'$ transitions in nuclei are suppressed due to kinematic reasons 
\cite{Berezhiani:2005hv}.  
On the other hand, 
existing experimental and astrophysical limits allow $n-n'$ oscillation to be 
a rather fast process, with the characteristic oscillation time $\tau_{nn'} = 1/\epsilon_{nn'}$  
much smaller than the neutron lifetime, with interesting 
implications for cosmic rays \cite{Berezhiani:2006je, Berezhiani:2011da}  and 
neutron stars \cite{Goldman:2019dbq,Berezhiani:2020zck,Berezhiani:2021src,Goldman:2022brt}. 
Namely, the scale of underlying new physics inducing the mixed six-quark operators 
can be at TeV, $C_{B=1} \sim (1~\text{TeV})^{-5}$ 
(cosmological limits  \cite{Berezhiani:2005hv,Babu:2021mjg} 
do not exclude such a possibility),
in which case $n-n'$ mixing can be as large as $\epsilon_{nn'} \sim 1$~neV or so. 
 
 The phenomena of $n-n'$ oscillations can be experimentally searched via  neutron disappearance 
$n\to n'$ and regeneration $n\to n' \to n$ 
\cite{Berezhiani:2005hv,Pokotilovski:2006gq,Berezhiani:2017azg}. 
Such transitions can also be induced via the non-diagonal magnetic moment 
between $n$ and $n'$ states \cite{Berezhiani:2018qqw}. 
Several experiments were performed searching for $n-n'$ oscillation with the UCN   
\cite{Ban:2007tp,Serebrov:2007gw,Altarev:2009tg,Bodek:2009zz,Serebrov:2008her,Berezhiani:2017jkn,nEDM:2020ekj,Mohanmurthy:2022dbt},  
and, for a simplest scenario of the case mass degenerate $n-n'$ oscillation, 
an upper limit was set on the oscillation time, $\tau_{nn'} < 414$~s \cite{Serebrov:2007gw}. 
However, this limit becomes invalid if there is some mass splitting between $n$ and $n'$ 
or $n-n'$ oscillation is affected by the presence of mirror magnetic fields \cite{Berezhiani:2009ldq}. 
Interestingly, some of the above experiments show anomalous deviations  
\cite{Berezhiani:2012rq}  which will be critically tested in the new experiments 
\cite{Ayres:2021zbh,Addazi:2020nlz}.  

The phenomena of $n-\bar{n}$ and $n-n'$ mixings can have a common theoretical origin which unify $\Delta B=1$ and $\Delta B=2$ interactions \cite{Berezhiani:2005hv,Berezhiani:2015afa}. 
More generally, the four states $n$, $\bar n$, $n'$ and $\bar{n}'$ can be all mixed with each other.  
While the direct $n-\bar n$ mixing, i.e. the neutron Majorana mass, is strongly 
restricted by experimental limits,  $\epsilon_{n\bar n} < 10^{-24}$ eV or so, 
$n-n'$ and $n-\bar{n}'$ mixings can be both much larger. In this way,  
significant effects of $n-\bar{n}$ transition can be induced via the above mixings: 
namely, a neutron travelling to mirror world can return back as an antineutron 
\cite{Berezhiani:2020nzn}. The probability of induced  $n\to n'\bar{n}' \to \bar{n}$ 
transition can be many orders of magnitude larger than that of direct $n-\bar n$ 
oscillation, and this phenomenon can be experimentally tested
 in new experiments which can properly scan the range of the applied magnetic field 
 \cite{Yiu:2022faw}.   
 
 Experimental prospects at the ESS are the HIBEAM/NNBAR projects as discussed in Section~\ref{sec:nnbar}.

 
\subsubsection{Searches for extra fundamental interactions,  gravitational spectroscopy, Lorentz invariance tests}
\label{sec:theoryextra}

Fundamental interactions additional to gravitational, electromagnetic, weak and strong are assumed in many extensions of the SM. They can arise for various reasons, including the existence of additional elementary particles or dimensions of space, dark matter or energy hypotheses. The existence of additional bosons induces a spin-independent Yukawa-type interaction with a characteristic range that is inversely proportional to the boson mass. If heavy bosons are to be sought at high energies, weakly interacting light bosons would elude such detection techniques. An additional boson may even be massless \cite{Lee:1955PR}, which would violate the equivalence principle at large distances. Theories with extra large dimensions of space \cite{Rubakov:1983PLB136,Rubakov:1983PLB139,Viser:1985PLB,Arkani:1998PLB,Arkani:1999PRD,Antoniadis:1998PLB,Antoniadis:1990PLB} predict observable spin-independent interactions. The light dark matter hypothesis \cite{Fayet:2007PRD} favors them. Chameleon-type interactions \cite{Pignol:2015IJMPA} are intensively researched. The existence of axion-like particles would lead to the existence of spin-dependent extra interactions \cite{Antoniadis:2011CRP}. 

A generic functional form of a new spin-independent interactions is the one of a Yukawa-type interaction between two particles with masses $m_1$ and $m_2$ at a distance $r$: $V(r)=\alpha G m_1 m_2/r\cdot \exp(-r/\lambda)$, where $\lambda=\hbar/mc$, with the mass of the new boson $m$, is the Yukawa range of the new interaction. Here, $\alpha=1$ would mean that the new interaction is as strong as gravity for short ranges. The most simple functional form of a new spin-dependent short-range interaction between an unpolarized spin-1/2 particle (1) and a polarized spin 1/2 particle (2) at a distance $r$, mediated by a light pseudoscalar boson of mass $m$, is given by
\begin{equation}
V(r)=g_s^1 g_p^2 \hbar^2/(8\pi m_2) \cdot (\sigma_2\cdot \hat{r}) (1/r\lambda+1/r^2) \exp(-r/\lambda).
\end{equation}
Here, $g_s^1 g_p^2$ is the product of the relevant coupling coefficients for the interaction between particle 1 (unpolarized) and 2 (polarized),  $m_2$ and $\sigma_2$ are the mass and the spin of the polarized particle, and $\lambda=\hbar/mc$ being the Yukawa range as above. The Yukawa range and the mass $m$ of the new boson are used as free parameters in the analysis. Figure~\ref{SRfig:ShortRangeLimits} shows the present most constraining limits for both of those interactions in the relevant Yukawa range. Other properties or functional forms of new short-range interactions are discussed in \cite{Dobrescu:2006,Safranova:2018,Fadeev:2019}. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{SRLimits.pdf}
    \caption{Left: Current most constraining limits for new spin-independent short-range forces. The first experiment (red line, \cite{Heacock:2021}) uses free neutrons. At higher $\lambda$ ranges, other techniques and probes are more sensitive \cite{Mohideen:1998,Chen:2016,Lee:2020,Tan:2020}. Right: Current most constraining limits for new spin-dependent interactions. Experiments \cite{Voronin:2009,Guigue:2015,Tullney:2013,Bulatowicz:2013} use the neutron as the polarized particle, for the first of those it is a free neutron. In \cite{Rong:2018, Hoedl:2011}, the polarized particle is an electron.}
    \label{SRfig:ShortRangeLimits}
\end{figure}

The large number of ways to search for extra interactions is reflected in the amount of data collected by the Particle Data Group \cite{Zyla:2020zbs}, e.g., in the review about ''Axions and other similar particles''. Depending on the type and range of extra interactions, neutrons play a unique or competitive role in this set of methods complementing searches at high-energy particle accelerators, in atoms, in low-background neutrino detectors, in searches for interactions on top of the van der Waals/Casimir-Polder interaction, measurements of gravity at short distances, astrophysical and cosmological constraints, and others. Several neutron experimental methods are available for such research, including neutron gravitational quantum spectroscopy \cite{Nes2002,Nesvizhevsky:2006,Jenke:2011NatP,Jenke:2014PRL,Cronenberg:NatP2018}, neutron scattering and interferometry \cite{Haddock:2018prd,Kamiya:2015, Snow:PRD,Guillaume:PLB,Nesvizhevsky:2009NatP,Brax:2018}, crystal neutron diffraction \cite{Heacock:2021,Voronin:2009,Voronin:2020}, neutron spin rotation \cite{Yan:2013,Haddock:2018plb}, and others. They allow also testing Lorentz invariance \cite{Martin:2018PRD,Escobar:2019PRD,Ivanov:2019PLB}, non-commutative quantum mechanics \cite{Bertolami:2009PRD,Saha:2007EPJC}, extensions of gravitational theories and many others. 

ESS can play a unique role among neutron sources if the experimental methods critically use the pulsed structure of ESS neutron fluxes, or unique ESS sources that can provide intense neutron fluxes with wavelengths unavailable today. In particular, this refers to the possibility of constructing an intense source of very cold neutrons. A broad window of opportunity for neutron experiments is open to constrain new interactions in the nanometer range and below, where neutrons are the best or competitive; the sensitivity of neutron experiments is rapidly improving for ranges up to about several micrometers, and is competitive for a number of scenarios. 
A distinct advantage of the neutron as a test particle is the absence of an electric charge and a small magnetic moment, respectively, and therefore the smallness of systematic effects. An important drawback is the low neutron flux, especially for neutrons with wavelengths optimal for these experiments. The ESS can remove precisely the most critical of the limitations of these experiments and allow a major increase in sensitivity, promising discovery potential. More details on ESS expectations are in the experimental Section~\ref{sec:ANNIneutroncharge}.% and~\ref{sec:neutroninterferometry}.

\subsubsection{Studies of hadronic parity violation}
\label{sec:theoryhpv}

%Nucleon-nucleon (NN) weak interaction amplitudes provide a very interesting ``computational frontier'' of the Standard Model. The relative sizes of different quark-quark weak interaction amplitudes, which in turn induce NN weak interactions, are very sensitive to quark-quark correlations in the nucleon and to low energy non-perturbative NN strong interaction dynamics. 

%The measurement of 
Nucleon nucleon (NN) weak amplitudes 
%therefore 
offer a unique, dynamically-rich regime in which to test the standard electroweak model.  
NN weak interactions provide a new opportunity to develop theoretical methods in low energy strong interaction theory such as effective field theory~\cite{Zhu:2004vw,deVries:2015gea} and lattice gauge theory~\cite{Wasem:2011tp}  and make predictions 
%(rather than post-dictions) 
in a challenging but calculable system~\cite{Adelberger:1985ik,Desplanques:1998ak,RamseyMusolf:2006dz,Haxton:2013aca,Schindler:2013yua,Gardner:2017xyl}, a recent review is \cite{deVries:2020iea}. The NN weak interaction is also a test case for our ability to trace symmetry-violating effects of a known quark-quark interaction 
in nuclei, 
%across many nonperturbative strong interaction scales, 
which is of great interest also for 
%other nuclear probes of new physics such as  
electric dipole moments and neutrinoless double beta decay.
%This is an exercise that also must be performed for many other searches for symmetry-violating low energy nuclear observables beyond the standard model such as electric dipole moments and neutrinoless double beta decay. 
NN weak interactions will soon become experimentally accessible due to recent advances in atomic and molecular optics (AMO) physics through the effects of parity-odd nuclear anapole moments~\cite{Flambaum:1980sb,Wood:1997zq,Tsigutkin:2009zz,Roberts:2014bka,Safronova:2017xyt,Wieman:2019vik} on atomic and molecular structure. Advances in laser cooling also allow to detect other effects via mixing of opposite-parity states in molecules~\cite{Hutzler:2020pze,Flambaum:1984xu,DeMille:2008,Altuntas:2018ots,Norrgard:2018uba}.
%Improved understanding of NN weak interaction in nuclei will also benefit planned searches for time reversal invariance in polarized neutron-nucleus optics~\cite{Mitchell:1999zz,Tomsovic:1999yb,Bowman:2014fca}. 
 
 
The value of the ESS for this physics lies in its unparalleled combination of high intensity slow neutron beams, needed to reach the statistical accuracy to see NN weak effects, and neutron energy information using neutron time of flight from this pulsed neutron source, 
%which 
%we know from experience  is very important 
needed for the suppression of systematic errors. The experimental aspects are discussed in Section~\ref{sec:ANNIHWI}.
%for the   ppb-level sensitivity to parity-odd asymmetries 
%
%needed to see NN weak interaction effects in the presence of the strong 
%interaction. 

Examples of possible NN weak experiments which can take special advantage of the strengths of the ESS are: (1) neutron-proton parity-odd spin rotation, which can access the $\Delta I=2$ NN weak amplitude that can most easily be calculated in lattice gauge theory,  (2) parity-odd gamma asymmetry in $\vec{n}+D \to T+\gamma$, which is a sufficiently simple system to be treatable using effective field theory techniques in terms of two-body NN weak amplitudes, (3) a remeasurement of the parity-odd gamma asymmetry in $\vec{n}+p \to D+\gamma$ recently measured at the Spallation Neutron Source (SNS) at ORNL ~\cite{Blyth:2018aon}, which can determine the very important weak pion exchange amplitude with higher precision, and (4) a repeat of the $\vec{n}+{}^3He \to {}^3H+p$ parity violation experiment, which was also recently measured at the SNS~\cite{McCrea:2020www} and can be done with higher precision.
 

\subsection{Neutrinos}
The ESS will provide the largest pulsed neutrino flux, opening unprecedented opportunities to study their interaction with matter and oscillations. The main theory aspects are introduced in this section, whereas experimental details will be discussed in Sections~\ref{sec:nuess} and~\ref{sec:ESSnuSB}.

\subsubsection{Coherent neutrino-nucleus scattering}
\label{sec:theoryneutrinoscattering}

In the SM neutrinos interact with matter not only through charged current but also through neutral current %(NC) 
via the tree-level exchange of a $Z$ boson. Interestingly enough at low energies the neutrino cannot resolve the nucleus, i.e., the neutrino interacts coherently with all the nucleons in the atomic nuclei, with the resulting enhancement in the cross section~\cite{Freedman:1973yd}. The challenging detection of the experimental signal of this Coherent Elastic Neutrino-Nucleus Scattering (CE$\nu$NS) was recently achieved by the COHERENT collaboration at the Oak Ridge National Laboratory~\cite{Akimov:2017ade}, opening exciting opportunities both at the technological and scientific levels.  

The ESS is particularly well suited for this kind of measurements thanks to its very high yield of low-energy neutrinos, which will allow for high-statistics measurements~\cite{Baxter:2019mcx}. It is worth noting that the use of multiple targets would allow us to disentangle various physics effects. These are discussed more in Section~\ref{sec:nuess}.

Concerning fundamental physics, CE$\nu$NS measurements offer interesting information about the nuclear structure of the target, such as the nuclear neutron distribution. Moreover, once such effects are properly parameterized, CE$\nu$NS measurements represent a unique probe of the interactions between neutrinos and quarks. Some applications include the extraction of the weak mixing angle at very low momentum transfer, the study of the neutrino electromagnetic properties and the search of non-standard interactions and new light particles (sterile neutrino, dark matter, etc)~\cite{Baxter:2019mcx}. More details about the experimental opportunities are in Section~\ref{sec:nuess}.
    




\subsubsection{Neutrino oscillations, leptonic CP violation, non-standard neutrino interactions with matter}
\label{sec:theoryneutrinooscillations}

The quantum mechanical phenomenon of neutrino oscillations has been experimentally observed by several different so-called neutrino oscillations experiments, including the Super-Kamiokande and SNO experiments \cite{Fukuda:1998mi,Ahmad:2002jz}. In the past decades, using data from atmospheric, solar, accelerator, and reactor neutrino experiments, the various parameters that describe neutrino oscillations have been measured to excellent precision. These parameters are two mass-squared differences $|\Delta m_{31}^2|$ and $\Delta m_{21}^2$ as well as three leptonic mixing angles $\theta_{12}$, $\theta_{13}$, and $\theta_{23}$.
Nevertheless, at the moment, at least three parameters remain to be determined, i.e. the mass ordering of neutrinos, the octant of the mixing angle $\theta_{23}$, and most importantly, the leptonic CP-violating phase $\delta_{\rm CP}$. Presently, there are many dedicated proposed experiments in order to measure these parameters.

The ESSnuSB \cite{Baussan:2013zcy,Wildner:2015yaa} is a proposed experiment at the ESS. Its main aim is to discover and measure leptonic CP violation, i.e., to determine the leptonic CP-violation phase $\delta_{\rm CP}$, with unprecedented sensitivity and related to that the matter-antimatter asymmetry of the Universe. Due to the fact that the leptonic mixing angle $\theta_{13}$ is unexpectely large, the ESSnuSB is optimal for obtaining maximal sensitivity in measuring leptonic CP violation at the so-called second neutrino oscillation maximum, see for example Refs.~\cite{Huber:2005jk,Huber:2010dx,Coloma:2011pg,Coloma:2014kca}. Currently, there are two different baseline lengths that are under investigation: 360 km (Zinkgruvan, Sweden) and 540 km (Garpenberg, Sweden), which are both situated at distances from the ESS that are suitable to the second neutrino oscillation maximum. During 2018--2021, the ESSnuSB has been investigated by a European Design Study project financed by the European Commission by its Horizon 2020 Framework Programme. Comparative studies between the ESSnuSB and other proposed experimental setups in determining the leptonic CP-violating phase have been carried out \cite{Chakraborty:2017ccm,Chakraborty:2019jlv,Ghosh:2019sfi}. It has also been argued \cite{Blennow:2019bvl} that the choice of the second neutrino oscillation maximum could reduce statistics and make complementary searches of e.g. the octant of $\theta_{23}$ less fruitful, thus opting for shorter baselines (such as the baseline length of the Zinkgruvan choice).

What is the difference between the first and the second neutrino oscillation maxima? For vacuum neutrino oscillations, the first oscillation maximum is defined as $|\Delta m_{31}^2| L/(4E) = \pi/2$, where $L$ is the length of the baseline and $E$ is the average neutrino energy, whereas the second oscillation maximum is given by $| \Delta m_{31}^2 | L/(4E) = 3 \pi/2$. Using the characteristic values of the ESSnuSB ($E \simeq 0.36$~GeV), we find that the first and second oscillation maxima are situated at $\hat{L}_1 \simeq 180$~km and $\hat{L}_2 \simeq 530$~km, respectively, for $\Delta m_{31}^2 = 2.5 \cdot 10^{-3} \, {\rm eV}^2$ \cite{Esteban:2020cvm}. Indeed, the value of second oscillation maximum is close to the baseline length of the Garpenberg choice (of the detector). It should be noted that taking into consideration matter effects and three-flavor neutrino oscillations, the definition of the neutrino oscillation maxima will change quantitatively, but not qualitatively.

In addition to measuring leptonic CP-violation, the ESSnuSB is an ideal experimental setup to investigate other new physics scenarios such as non-standard neutrino interactions, sterile neutrino, and neutrino decay. For recent reviews on, for example, non-standard neutrino interactions, see Refs.~\cite{Ohlsson:2012kf,Miranda:2015dra,Farzan:2017xzy}. In phenomenological studies, so-called source and detector non-standard neutrino interactions have been explored \cite{Blennow:2015nxa}, the sensitivity to light sterile neutrinos has been studied \cite{Agarwalla:2019zex,Ghosh:2019zvl}, and the search and possibility of invisible neutrino decay has been investigated \cite{Blennow:2014fqa,Choubey:2020dhw,Chakraborty:2020cfu}. Furthermore, it has been proposed to use the ESSnuSB to test lepton flavor models \cite{Blennow:2020snb,Blennow:2020ncm}. Such models, which give rise to a non-zero leptonic Dirac CP-violating phase, could be related to the matter-antimatter asymmetry of the Universe \cite{Bertuzzo:2009im,Chen:2016ptr,Hagedorn:2016lva} and are basically testable with the ESSnuSB. In comparative studies, the ESSnuSB has also been used to put stringent constraints on fundamental symmetries such as potential CPT violation in neutrino oscillations \cite{Ohlsson:2014cha,Majhi:2021api}. The experimental aspects of ESSnuSB are discussed in Section~\ref{sec:ESSnuSB}.
<
